Learning with Hierarchical Gaussian Kernels

We investigate iterated compositions of weighted sums of Gaussian kernels and provide an interpretation of the construction that shows some similarities with the architectures of deep neural networks. On the theoretical side, we show that these kernels are universal and that SVMs using these kernels are universally consistent. We further describe a parameter optimization method for the kernel parameters and empirically compare this method to SVMs, random forests, a multiple kernel learning approach, and to some deep neural networks.

==> data-table.tex <==
\begin{table}
\begin{center}
{
{\footnotesize
\begin{tabular}{|r|r|r|r|r|r|r|}
\hline
Data Set &  Size & Dim. & Type & Train. & Extra &Source\\
\hline
{\sc Bank-Marketing}  &  45211  &  16   &  BC & 7000 & 14000 & UCI \\
\hline
{\sc Cadata*}  & 20640   &   8  & REG &  7000 & 7000 & LIBSVM \\
\hline
{\sc Cod-rna}  & 331152   &  8   &  BC & 7000 & 14000& LIBSVM \\
\hline
{\sc Covtype}  & 581012   & 55    &  BC & 7000& 14000& UCI \\
\hline
{\sc Cpusmall}  &  8192  &  12   & REG &  6000& 0 & LIBSVM \\
\hline
{\sc Cycle-Power-Plant}  &  9568  &  4   & REG & 6000 & 0  & UCI \\
\hline
{\sc Higgs*}  &  50000  &  28   &   BC &7000 & 14000 & UCI \\
\hline
{\sc Letter-Recognition}  &  20000  &  16   & MC-26 & 7000& 7000&  UCI   \\
\hline
{\sc Magic}  & 19020   &   10  & BC & 7000 & 7000 & UCI   \\
\hline
{\sc Pendigits}  & 10992   &  16   & MC-10 & 7000 & 0 & UCI  \\
\hline
{\sc Satimage}  & 6435   &   36  &  MC-6  & 5000 & 0 & UCI\\
\hline
{\sc Seismic}  &  98528  & 50  & MC-3  & 7000 & 14000 & LIBSVM   \\
\hline
{\sc Shuttle*}  &  43500  & 8    & MC-6 & 7000 & 14000 & LIBSVM    \\
\hline
{\sc Thyroid-ann}  & 7200   &  21   &  BC & 5000 & 0 & UCI \\
\hline
{\sc Updrs-motor}  & 5875   &  19   &  REG & 5000 & 0 & UCI \\
\hline
\end{tabular}
}
}
\end{center}
\caption{{\small Details of the considered datasets and their preparation. All data sets were scaled 
to either $[-1,1]$ or $[0,1]$. In addition, the ones marked by a $*$ were further modified as follows:
For {\sc Cadata} we scaled the labels by $0.0001$ to report comparable test errors, for {\sc Higgs}
we only considered a subsample of the specified size, and for {\sc Shuttle} we removed the first 
data column that contains a time stamp whose influence has been debated in the literature.
The types are binary classification (BC), regression (REG), and multiclass classification with $x$ labels
(MC-$x$). We subsampled a training set of the specified size, and for the larger data sets an 
additional subset (Extra column). All remaining samples were used for testing. These splits into two 
or three subsets were ten times repeated.
}}
\label{data-table}
\end{table}

==> fnew_experiments.tex <==
\begin{tabular}{|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
Data Set &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}1, S\hspace*{0.2ex}=\hspace*{0.2ex}1\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}1, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}1, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}1, S\hspace*{0.2ex}=\hspace*{0.2ex}6\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}1\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}6\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}1\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}6\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}1\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}6\!\!& \!best Arch.\!& Gauss \\
\hline
\!\!{\sc bank}\!\!&\!\!0.292 {\tiny $\pm$\hspace*{0.2ex}.005}\!\! & --- & --- & --- & ---&\!\!0.275 {\tiny $\pm$\hspace*{0.2ex}.013}\!\!&\!\!0.273 {\tiny $\pm$\hspace*{0.2ex}.009}\!\! & --- & ---&\!\!0.280 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.269 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!\textbf{0.266} {\tiny $\pm$\hspace*{0.2ex}.009}\!\! & ---&\!\!0.281 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.277 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!0.268 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! & ---&\!\!0.298 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc cadata}\!\!&\!\!.0538 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & --- & --- & --- & ---&\!\!.0540 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0538 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & --- & ---&\!\!.0534 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0536 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0533 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & ---&\!\!.0523 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!\textbf{.0522} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0525 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! & ---&\!\!.0545 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc cod}\!\!&\!\!0.144 {\tiny $\pm$\hspace*{0.2ex}.004}\!\! & --- & --- & --- & ---&\!\!0.131 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!0.135 {\tiny $\pm$\hspace*{0.2ex}.005}\!\! & --- & ---&\!\!0.132 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!0.133 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!0.134 {\tiny $\pm$\hspace*{0.2ex}.005}\!\! & ---&\!\!\textbf{0.131} {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.134 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!0.137 {\tiny $\pm$\hspace*{0.2ex}.006}\!\! & ---&\!\!0.158 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc covtype}\!\!&\!\!0.407 {\tiny $\pm$\hspace*{0.2ex}.013}\!\! & --- & --- & --- & ---&\!\!0.416 {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!\textbf{0.405} {\tiny $\pm$\hspace*{0.2ex}.015}\!\! & --- & ---&\!\!0.426 {\tiny $\pm$\hspace*{0.2ex}.019}\!\!&\!\!0.413 {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!0.411 {\tiny $\pm$\hspace*{0.2ex}.016}\!\! & ---&\!\!0.450 {\tiny $\pm$\hspace*{0.2ex}.021}\!\!&\!\!0.414 {\tiny $\pm$\hspace*{0.2ex}.024}\!\!&\!\!0.425 {\tiny $\pm$\hspace*{0.2ex}.021}\!\! & ---&\!\!0.520 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc cpusmall}\!\!&\!\!.0035 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & --- & --- & --- & ---&\!\!\textbf{.0033} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0034 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & --- & ---&\!\!.0033 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0033 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0034 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & ---&\!\!.0034 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0033 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0033 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & ---&\!\!.0036 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! \\
\hline
\!\!{\sc cycle}\!\!&\!\!.0103 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & --- & --- & --- & ---&\!\!.0101 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0102 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & --- & ---&\!\!.0101 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0101 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0101 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & --- & ---&\!\!.0102 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{.0100} {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & ---&\!\!.0106 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! \\
\hline
\!\!{\sc higgs}\!\!&\!\!0.808 {\tiny $\pm$\hspace*{0.2ex}0.24}\!\! & --- & --- & --- & ---&\!\!0.767 {\tiny $\pm$\hspace*{0.2ex}0.22}\!\!&\!\!0.749 {\tiny $\pm$\hspace*{0.2ex}0.22}\!\! & --- & ---&\!\!0.786 {\tiny $\pm$\hspace*{0.2ex}0.23}\!\!&\!\!\textbf{0.744} {\tiny $\pm$\hspace*{0.2ex}0.22}\!\!&\!\!0.750 {\tiny $\pm$\hspace*{0.2ex}0.22}\!\! & ---&\!\!0.795 {\tiny $\pm$\hspace*{0.2ex}0.23}\!\!&\!\!0.769 {\tiny $\pm$\hspace*{0.2ex}0.22}\!\!&\!\!0.766 {\tiny $\pm$\hspace*{0.2ex}0.23}\!\! & ---&\!\!0.833 {\tiny $\pm$\hspace*{0.2ex}0.25}\!\! \\
\hline
\!\!{\sc letter}\!\!&\!\!.0361 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! & --- & --- & --- & ---&\!\!.0354 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0344 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & --- & ---&\!\!.0355 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!\textbf{.0343} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0346 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & ---&\!\!.0354 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0343 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0347 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & ---&\!\!.0452 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc magic}\!\!&\!\!0.396 {\tiny $\pm$\hspace*{0.2ex}.007}\!\! & --- & --- & --- & ---&\!\!0.389 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.395 {\tiny $\pm$\hspace*{0.2ex}.009}\!\! & --- & ---&\!\!0.388 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!\textbf{0.386} {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.393 {\tiny $\pm$\hspace*{0.2ex}.006}\!\! & ---&\!\!0.387 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.390 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.390 {\tiny $\pm$\hspace*{0.2ex}.007}\!\! & ---&\!\!0.398 {\tiny $\pm$\hspace*{0.2ex}.007}\!\! \\
\hline
\!\!{\sc pendigits}\!\!&\!\!.0075 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & --- & --- & --- & ---&\!\!.0072 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0075 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & --- & ---&\!\!.0072 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0072 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0072 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & ---&\!\!\textbf{.0071} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0072 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0072 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & ---&\!\!.0081 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc satimage}\!\!&\!\!.0482 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & --- & --- & --- & ---&\!\!.0458 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0455 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & --- & ---&\!\!.0471 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0456 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!\textbf{.0449} {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & ---&\!\!.0471 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0462 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0458 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & ---&\!\!.0482 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc seismic}\!\!&\!\!0.307 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & --- & --- & --- & ---&\!\!0.299 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.299 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! & --- & ---&\!\!0.300 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.299 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.299 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & ---&\!\!0.300 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.299 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!\textbf{0.298} {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & ---&\!\!0.311 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc shuttle}\!\!&\!\!\textbf{.0041} {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & --- & --- & --- & ---&\!\!.0047 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0044 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & --- & ---&\!\!.0054 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0047 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0045 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & ---&\!\!.0066 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0055 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0051 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & ---&\!\!.0046 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! \\
\hline
\!\!{\sc thyroid}\!\!&\!\!\textbf{0.153} {\tiny $\pm$\hspace*{0.2ex}.009}\!\! & --- & --- & --- & ---&\!\!0.155 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!0.160 {\tiny $\pm$\hspace*{0.2ex}.009}\!\! & --- & ---&\!\!0.153 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.161 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!0.163 {\tiny $\pm$\hspace*{0.2ex}.009}\!\! & ---&\!\!0.153 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!0.156 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!0.159 {\tiny $\pm$\hspace*{0.2ex}.009}\!\! & ---&\!\!0.173 {\tiny $\pm$\hspace*{0.2ex}.009}\!\! \\
\hline
\!\!{\sc updrs}\!\!&\!\!.0118 {\tiny $\pm$\hspace*{0.2ex}.012}\!\! & --- & --- & --- & ---&\!\!\textbf{.0099} {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!.0129 {\tiny $\pm$\hspace*{0.2ex}.010}\!\! & --- & ---&\!\!.0319 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!.0184 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!.0176 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! & ---&\!\!.0361 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!.0146 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!.0107 {\tiny $\pm$\hspace*{0.2ex}.004}\!\! & ---&\!\!.0530 {\tiny $\pm$\hspace*{0.2ex}.004}\!\! \\
\hline 
\end{tabular}



==> initial_experiments-rerun.tex <==
\begin{tabular}{|r|r|r|r|r|r|r|r|r|}
\hline
Data Set &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\!& \!best Arch.\!& Gauss \\
\hline
\!\!{\sc bank}\!\!&\!\!\textbf{.0675} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0721 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0698 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0689 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0699 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0681 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & ---&\!\!.0754 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc cadata}\!\!&\!\!31.28 {\tiny $\pm$\hspace*{0.2ex}0.41}\!\!&\!\!29.41 {\tiny $\pm$\hspace*{0.2ex}0.56}\!\!&\!\!\textbf{27.07} {\tiny $\pm$\hspace*{0.2ex}0.46}\!\!&\!\!31.25 {\tiny $\pm$\hspace*{0.2ex}0.89}\!\! & ---&\!\!31.45 {\tiny $\pm$\hspace*{0.2ex}0.93}\!\! & ---&\!\!32.38 {\tiny $\pm$\hspace*{0.2ex}0.76}\!\! \\
\hline
\!\!{\sc cod}\!\!&\!\!0.169 {\tiny $\pm$\hspace*{0.2ex}.006}\!\!&\!\!\textbf{0.139} {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!0.152 {\tiny $\pm$\hspace*{0.2ex}.006}\!\!&\!\!0.178 {\tiny $\pm$\hspace*{0.2ex}.007}\!\! & ---&\!\!0.181 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & ---&\!\!0.188 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc covtype}\!\!&\!\!0.423 {\tiny $\pm$\hspace*{0.2ex}.013}\!\!&\!\!0.416 {\tiny $\pm$\hspace*{0.2ex}.015}\!\!&\!\!\textbf{0.404} {\tiny $\pm$\hspace*{0.2ex}.012}\!\!&\!\!0.424 {\tiny $\pm$\hspace*{0.2ex}.027}\!\!&\!\!0.480 {\tiny $\pm$\hspace*{0.2ex}.020}\!\!&\!\!0.410 {\tiny $\pm$\hspace*{0.2ex}.019}\!\! & ---&\!\!0.527 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc cpusmall}\!\!&\!\!8.745 {\tiny $\pm$\hspace*{0.2ex}0.26}\!\!&\!\!\textbf{8.553} {\tiny $\pm$\hspace*{0.2ex}0.36}\!\!&\!\!8.877 {\tiny $\pm$\hspace*{0.2ex}0.30}\!\!&\!\!8.701 {\tiny $\pm$\hspace*{0.2ex}0.20}\!\! & ---&\!\!8.600 {\tiny $\pm$\hspace*{0.2ex}0.38}\!\! & ---&\!\!9.263 {\tiny $\pm$\hspace*{0.2ex}0.29}\!\! \\
\hline
\!\!{\sc cycle}\!\!&\!\!\textbf{11.97} {\tiny $\pm$\hspace*{0.2ex}3.33}\!\!&\!\!14.05 {\tiny $\pm$\hspace*{0.2ex}0.78}\!\! & ---&\!\!12.52 {\tiny $\pm$\hspace*{0.2ex}1.61}\!\! & --- & --- & ---&\!\!14.74 {\tiny $\pm$\hspace*{0.2ex}0.50}\!\! \\
\hline
\!\!{\sc higgs}\!\!&\!\!0.819 {\tiny $\pm$\hspace*{0.2ex}.028}\!\!&\!\!\textbf{0.811} {\tiny $\pm$\hspace*{0.2ex}.020}\!\!&\!\!0.845 {\tiny $\pm$\hspace*{0.2ex}.029}\!\!&\!\!0.849 {\tiny $\pm$\hspace*{0.2ex}.023}\!\!&\!\!0.848 {\tiny $\pm$\hspace*{0.2ex}.026}\!\!&\!\!0.822 {\tiny $\pm$\hspace*{0.2ex}.033}\!\! & ---&\!\!0.905 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc letter}\!\!&\!\!5.645 {\tiny $\pm$\hspace*{0.2ex}0.32}\!\!&\!\!5.644 {\tiny $\pm$\hspace*{0.2ex}0.40}\!\!&\!\!5.748 {\tiny $\pm$\hspace*{0.2ex}0.27}\!\!&\!\!5.599 {\tiny $\pm$\hspace*{0.2ex}0.31}\!\!&\!\!5.848 {\tiny $\pm$\hspace*{0.2ex}0.31}\!\!&\!\!\textbf{5.583} {\tiny $\pm$\hspace*{0.2ex}0.33}\!\! & ---&\!\!7.158 {\tiny $\pm$\hspace*{0.2ex}0.31}\!\! \\
\hline
\!\!{\sc magic}\!\!&\!\!.0993 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0999 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0990 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{.0977} {\tiny $\pm$\hspace*{0.2ex}.002}\!\! & ---&\!\!.0990 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & ---&\!\!0.103 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc pendigits}\!\!&\!\!0.177 {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!0.214 {\tiny $\pm$\hspace*{0.2ex}.018}\!\!&\!\!0.160 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!0.177 {\tiny $\pm$\hspace*{0.2ex}.012}\!\!&\!\!\textbf{0.160} {\tiny $\pm$\hspace*{0.2ex}.013}\!\!&\!\!0.160 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! & ---&\!\!0.170 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! \\
\hline
\!\!{\sc satimage}\!\!&\!\!1.840 {\tiny $\pm$\hspace*{0.2ex}1.61}\!\!&\!\!0.827 {\tiny $\pm$\hspace*{0.2ex}.057}\!\!&\!\!\textbf{0.565} {\tiny $\pm$\hspace*{0.2ex}.045}\!\!&\!\!2.467 {\tiny $\pm$\hspace*{0.2ex}1.76}\!\!&\!\!0.639 {\tiny $\pm$\hspace*{0.2ex}.056}\!\!&\!\!0.802 {\tiny $\pm$\hspace*{0.2ex}0.11}\!\! & ---&\!\!4.898 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc seismic}\!\!&\!\!0.302 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!\textbf{0.298} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.304 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.301 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.303 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.301 {\tiny $\pm$\hspace*{0.2ex}.004}\!\! & ---&\!\!0.318 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc shuttle}\!\!&\!\!.0482 {\tiny $\pm$\hspace*{0.2ex}.007}\!\!&\!\!\textbf{.0465} {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!.0684 {\tiny $\pm$\hspace*{0.2ex}.006}\!\!&\!\!.0513 {\tiny $\pm$\hspace*{0.2ex}.004}\!\! & ---&\!\!.0521 {\tiny $\pm$\hspace*{0.2ex}.005}\!\! & ---&\!\!.0471 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc thyroid}\!\!&\!\!0.154 {\tiny $\pm$\hspace*{0.2ex}.012}\!\!&\!\!\textbf{0.153} {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.159 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!0.156 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.157 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.155 {\tiny $\pm$\hspace*{0.2ex}.005}\!\! & ---&\!\!0.195 {\tiny $\pm$\hspace*{0.2ex}.014}\!\! \\
\hline
\!\!{\sc updrs}\!\!&\!\!.0193 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!.0339 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!.0249 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!\textbf{.0070} {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0387 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0112 {\tiny $\pm$\hspace*{0.2ex}.007}\!\! & ---&\!\!.0530 {\tiny $\pm$\hspace*{0.2ex}.004}\!\! \\
\hline 
\end{tabular}



==> initial_experiments.tex <==
\begin{tabular}{|r|r|r|r|r|r|r|r|r|}
\hline
Data Set &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\!& \!best Arch.\!& Gauss \\
\hline
\!\!{\sc bank}\!\!&\!\!\textbf{.0694} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0719 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0722 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0699 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0713 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0704 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{\textit{.0680}} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0754 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc cadata}\!\!&\!\!31.56 {\tiny $\pm$\hspace*{0.2ex}0.40}\!\!&\!\!29.69 {\tiny $\pm$\hspace*{0.2ex}0.46}\!\!&\!\!\textbf{27.33} {\tiny $\pm$\hspace*{0.2ex}0.71}\!\!&\!\!31.41 {\tiny $\pm$\hspace*{0.2ex}0.56}\!\! & ---&\!\!31.58 {\tiny $\pm$\hspace*{0.2ex}0.78}\!\!&\!\!\textbf{\textit{27.33}} {\tiny $\pm$\hspace*{0.2ex}0.71}\!\!&\!\!32.38 {\tiny $\pm$\hspace*{0.2ex}0.76}\!\! \\
\hline
\!\!{\sc cod}\!\!&\!\!0.170 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!\textbf{0.142} {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.154 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!0.181 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & ---&\!\!0.181 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.142 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!0.188 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc covtype}\!\!&\!\!0.415 {\tiny $\pm$\hspace*{0.2ex}.018}\!\!&\!\!\textbf{0.414} {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.426 {\tiny $\pm$\hspace*{0.2ex}.023}\!\!&\!\!0.421 {\tiny $\pm$\hspace*{0.2ex}.019}\!\!&\!\!0.448 {\tiny $\pm$\hspace*{0.2ex}.023}\!\!&\!\!0.432 {\tiny $\pm$\hspace*{0.2ex}.032}\!\!&\!\!\textbf{\textit{0.409}} {\tiny $\pm$\hspace*{0.2ex}.007}\!\!&\!\!0.527 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc cpusmall}\!\!&\!\!9.015 {\tiny $\pm$\hspace*{0.2ex}0.38}\!\!&\!\!\textbf{8.699} {\tiny $\pm$\hspace*{0.2ex}0.22}\!\!&\!\!8.750 {\tiny $\pm$\hspace*{0.2ex}0.28}\!\!&\!\!8.814 {\tiny $\pm$\hspace*{0.2ex}0.25}\!\! & ---&\!\!8.889 {\tiny $\pm$\hspace*{0.2ex}0.25}\!\! & ---&\!\!9.263 {\tiny $\pm$\hspace*{0.2ex}0.29}\!\! \\
\hline
\!\!{\sc cycle}\!\!&\!\!14.45 {\tiny $\pm$\hspace*{0.2ex}0.74}\!\!&\!\!14.24 {\tiny $\pm$\hspace*{0.2ex}0.76}\!\! & ---&\!\!\textbf{13.92} {\tiny $\pm$\hspace*{0.2ex}0.68}\!\! & --- & --- & ---&\!\!14.74 {\tiny $\pm$\hspace*{0.2ex}0.50}\!\! \\
\hline
\!\!{\sc higgs}\!\!&\!\!\textbf{0.819} {\tiny $\pm$\hspace*{0.2ex}.023}\!\!&\!\!0.833 {\tiny $\pm$\hspace*{0.2ex}.013}\!\!&\!\!0.867 {\tiny $\pm$\hspace*{0.2ex}.024}\!\!&\!\!0.832 {\tiny $\pm$\hspace*{0.2ex}.035}\!\!&\!\!0.869 {\tiny $\pm$\hspace*{0.2ex}.025}\!\!&\!\!0.859 {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!\textbf{\textit{0.810}} {\tiny $\pm$\hspace*{0.2ex}.015}\!\!&\!\!0.905 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc letter}\!\!&\!\!5.880 {\tiny $\pm$\hspace*{0.2ex}0.44}\!\!&\!\!5.864 {\tiny $\pm$\hspace*{0.2ex}0.45}\!\!&\!\!5.879 {\tiny $\pm$\hspace*{0.2ex}0.45}\!\!&\!\!\textbf{5.727} {\tiny $\pm$\hspace*{0.2ex}0.30}\!\!&\!\!5.998 {\tiny $\pm$\hspace*{0.2ex}0.23}\!\!&\!\!5.757 {\tiny $\pm$\hspace*{0.2ex}0.30}\!\!&\!\!5.755 {\tiny $\pm$\hspace*{0.2ex}0.33}\!\!&\!\!7.158 {\tiny $\pm$\hspace*{0.2ex}0.31}\!\! \\
\hline
\!\!{\sc magic}\!\!&\!\!0.101 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.100 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.100 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.100} {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & ---&\!\!0.100 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.100 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.103 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc pendigits}\!\!&\!\!0.179 {\tiny $\pm$\hspace*{0.2ex}.015}\!\!&\!\!0.203 {\tiny $\pm$\hspace*{0.2ex}.014}\!\!&\!\!\textbf{0.157} {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!0.179 {\tiny $\pm$\hspace*{0.2ex}.014}\!\!&\!\!0.164 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!0.159 {\tiny $\pm$\hspace*{0.2ex}.012}\!\! & ---&\!\!0.170 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! \\
\hline
\!\!{\sc satimage}\!\!&\!\!0.914 {\tiny $\pm$\hspace*{0.2ex}0.63}\!\!&\!\!0.910 {\tiny $\pm$\hspace*{0.2ex}0.18}\!\!&\!\!\textbf{0.610} {\tiny $\pm$\hspace*{0.2ex}.045}\!\!&\!\!0.681 {\tiny $\pm$\hspace*{0.2ex}.070}\!\!&\!\!0.639 {\tiny $\pm$\hspace*{0.2ex}.045}\!\!&\!\!0.714 {\tiny $\pm$\hspace*{0.2ex}.042}\!\! & ---&\!\!4.898 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc seismic}\!\!&\!\!0.301 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.298} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.304 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.303 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.304 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.305 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.300 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.318 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc shuttle}\!\!&\!\!.0500 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!\textbf{.0460} {\tiny $\pm$\hspace*{0.2ex}.007}\!\!&\!\!.0713 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!.0519 {\tiny $\pm$\hspace*{0.2ex}.006}\!\! & ---&\!\!.0521 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!.0479 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!.0471 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc thyroid}\!\!&\!\!0.161 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!\textbf{0.158} {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.166 {\tiny $\pm$\hspace*{0.2ex}.013}\!\!&\!\!0.158 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.165 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!0.163 {\tiny $\pm$\hspace*{0.2ex}.009}\!\! & ---&\!\!0.195 {\tiny $\pm$\hspace*{0.2ex}.014}\!\! \\
\hline
\!\!{\sc updrs}\!\!&\!\!.0301 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0409 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!.0267 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!\textbf{.0217} {\tiny $\pm$\hspace*{0.2ex}.012}\!\!&\!\!.0397 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0235 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! & ---&\!\!.0530 {\tiny $\pm$\hspace*{0.2ex}.004}\!\! \\
\hline 
\end{tabular}



==> initial_experiments_safe.tex <==
\begin{tabular}{|r|r|r|r|r|r|r|r|r|}
\hline
Data Set &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\!& \!best Arch.\!& Gauss \\
\hline
\!\!{\sc bank}\!\!&\!\!\textbf{.0694} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0719 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0722 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!\textbf{.0699} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0713 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0704 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{\textit{.0680}} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0754 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc cadata}\!\!&\!\!31.56 {\tiny $\pm$\hspace*{0.2ex}0.40}\!\!&\!\!29.69 {\tiny $\pm$\hspace*{0.2ex}0.46}\!\!&\!\!\textbf{27.33} {\tiny $\pm$\hspace*{0.2ex}0.71}\!\!&\!\!31.41 {\tiny $\pm$\hspace*{0.2ex}0.56}\!\! & ---&\!\!31.58 {\tiny $\pm$\hspace*{0.2ex}0.78}\!\!&\!\!\textbf{\textit{27.33}} {\tiny $\pm$\hspace*{0.2ex}0.71}\!\!&\!\!32.38 {\tiny $\pm$\hspace*{0.2ex}0.76}\!\! \\
\hline
\!\!{\sc cod}\!\!&\!\!0.170 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!\textbf{0.142} {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.154 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!0.181 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & ---&\!\!0.181 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.142 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!0.188 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc covtype}\!\!&\!\!0.415 {\tiny $\pm$\hspace*{0.2ex}.018}\!\!&\!\!\textbf{0.414} {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.426 {\tiny $\pm$\hspace*{0.2ex}.023}\!\!&\!\!0.421 {\tiny $\pm$\hspace*{0.2ex}.019}\!\!&\!\!0.448 {\tiny $\pm$\hspace*{0.2ex}.023}\!\!&\!\!0.432 {\tiny $\pm$\hspace*{0.2ex}.032}\!\!&\!\!\textbf{\textit{0.409}} {\tiny $\pm$\hspace*{0.2ex}.007}\!\!&\!\!0.527 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc cpusmall}\!\!&\!\!9.015 {\tiny $\pm$\hspace*{0.2ex}0.38}\!\!&\!\!\textbf{8.699} {\tiny $\pm$\hspace*{0.2ex}0.22}\!\!&\!\!8.750 {\tiny $\pm$\hspace*{0.2ex}0.28}\!\!&\!\!8.814 {\tiny $\pm$\hspace*{0.2ex}0.25}\!\! & ---&\!\!8.889 {\tiny $\pm$\hspace*{0.2ex}0.25}\!\! & ---&\!\!9.263 {\tiny $\pm$\hspace*{0.2ex}0.29}\!\! \\
\hline
\!\!{\sc cycle}\!\!&\!\!14.45 {\tiny $\pm$\hspace*{0.2ex}0.74}\!\!&\!\!14.24 {\tiny $\pm$\hspace*{0.2ex}0.76}\!\! & ---&\!\!\textbf{13.92} {\tiny $\pm$\hspace*{0.2ex}0.68}\!\! & --- & --- & ---&\!\!14.74 {\tiny $\pm$\hspace*{0.2ex}0.50}\!\! \\
\hline
\!\!{\sc higgs}\!\!&\!\!\textbf{0.819} {\tiny $\pm$\hspace*{0.2ex}.023}\!\!&\!\!0.833 {\tiny $\pm$\hspace*{0.2ex}.013}\!\!&\!\!0.867 {\tiny $\pm$\hspace*{0.2ex}.024}\!\!&\!\!0.832 {\tiny $\pm$\hspace*{0.2ex}.035}\!\!&\!\!0.869 {\tiny $\pm$\hspace*{0.2ex}.025}\!\!&\!\!0.859 {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!\textbf{\textit{0.810}} {\tiny $\pm$\hspace*{0.2ex}.015}\!\!&\!\!0.905 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc letter}\!\!&\!\!5.880 {\tiny $\pm$\hspace*{0.2ex}0.44}\!\!&\!\!5.864 {\tiny $\pm$\hspace*{0.2ex}0.45}\!\!&\!\!5.879 {\tiny $\pm$\hspace*{0.2ex}0.45}\!\!&\!\!\textbf{5.727} {\tiny $\pm$\hspace*{0.2ex}0.30}\!\!&\!\!5.998 {\tiny $\pm$\hspace*{0.2ex}0.23}\!\!&\!\!5.757 {\tiny $\pm$\hspace*{0.2ex}0.30}\!\!&\!\!5.755 {\tiny $\pm$\hspace*{0.2ex}0.33}\!\!&\!\!7.158 {\tiny $\pm$\hspace*{0.2ex}0.31}\!\! \\
\hline
\!\!{\sc magic}\!\!&\!\!0.101 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.100} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.100} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.100} {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & ---&\!\!\textbf{0.100} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{\textit{0.100}} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.103 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc pendigits}\!\!&\!\!0.179 {\tiny $\pm$\hspace*{0.2ex}.015}\!\!&\!\!0.203 {\tiny $\pm$\hspace*{0.2ex}.014}\!\!&\!\!\textbf{0.157} {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!0.179 {\tiny $\pm$\hspace*{0.2ex}.014}\!\!&\!\!0.164 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!0.159 {\tiny $\pm$\hspace*{0.2ex}.012}\!\! & ---&\!\!0.170 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! \\
\hline
\!\!{\sc satimage}\!\!&\!\!0.914 {\tiny $\pm$\hspace*{0.2ex}0.63}\!\!&\!\!0.910 {\tiny $\pm$\hspace*{0.2ex}0.18}\!\!&\!\!\textbf{0.610} {\tiny $\pm$\hspace*{0.2ex}.045}\!\!&\!\!0.681 {\tiny $\pm$\hspace*{0.2ex}.070}\!\!&\!\!0.639 {\tiny $\pm$\hspace*{0.2ex}.045}\!\!&\!\!0.714 {\tiny $\pm$\hspace*{0.2ex}.042}\!\! & ---&\!\!4.898 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc seismic}\!\!&\!\!0.301 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.298} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.304 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.303 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.304 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.305 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.300 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.318 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc shuttle}\!\!&\!\!.0500 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!\textbf{.0460} {\tiny $\pm$\hspace*{0.2ex}.007}\!\!&\!\!.0713 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!.0519 {\tiny $\pm$\hspace*{0.2ex}.006}\!\! & ---&\!\!.0521 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!.0479 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!.0471 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc thyroid}\!\!&\!\!0.161 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!\textbf{0.158} {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.166 {\tiny $\pm$\hspace*{0.2ex}.013}\!\!&\!\!\textbf{0.158} {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.165 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!0.163 {\tiny $\pm$\hspace*{0.2ex}.009}\!\! & ---&\!\!0.195 {\tiny $\pm$\hspace*{0.2ex}.014}\!\! \\
\hline
\!\!{\sc updrs}\!\!&\!\!.0301 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0409 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!.0267 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!\textbf{.0217} {\tiny $\pm$\hspace*{0.2ex}.012}\!\!&\!\!.0397 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0235 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! & ---&\!\!.0530 {\tiny $\pm$\hspace*{0.2ex}.004}\!\! \\
\hline 
\end{tabular}



==> new_experiments.tex <==
\begin{tabular}{|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
Data Set &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}1, S\hspace*{0.2ex}=\hspace*{0.2ex}1\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}6\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}6\!\!& Gauss \\
\hline
\!\!{\sc bank}\!\!&\!\!0.290 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!0.274 {\tiny $\pm$\hspace*{0.2ex}.012}\!\!&\!\!0.272 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.276 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!0.269 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!\textbf{0.266} {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.280 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.277 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!0.267 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!0.298 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc cadata}\!\!&\!\!.0531 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0533 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0531 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0528 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0529 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0526 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0518 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!\textbf{.0516} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0518 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0538 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc cod}\!\!&\!\!0.144 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!0.132 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!0.134 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!0.131 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!0.132 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!0.133 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!\textbf{0.130} {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.134 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!0.135 {\tiny $\pm$\hspace*{0.2ex}.006}\!\!&\!\!0.157 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc covtype}\!\!&\!\!0.417 {\tiny $\pm$\hspace*{0.2ex}.017}\!\!&\!\!0.421 {\tiny $\pm$\hspace*{0.2ex}.024}\!\!&\!\!\textbf{0.406} {\tiny $\pm$\hspace*{0.2ex}.015}\!\!&\!\!0.424 {\tiny $\pm$\hspace*{0.2ex}.021}\!\!&\!\!0.419 {\tiny $\pm$\hspace*{0.2ex}.022}\!\!&\!\!0.416 {\tiny $\pm$\hspace*{0.2ex}.019}\!\!&\!\!0.445 {\tiny $\pm$\hspace*{0.2ex}.023}\!\!&\!\!0.418 {\tiny $\pm$\hspace*{0.2ex}.026}\!\!&\!\!0.426 {\tiny $\pm$\hspace*{0.2ex}.022}\!\!&\!\!0.521 {\tiny $\pm$\hspace*{0.2ex}.004}\!\! \\
\hline
\!\!{\sc cpusmall}\!\!&\!\!.0036 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{.0033} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0034 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0034 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0034 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0034 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0034 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0034 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0034 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0036 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! \\
\hline
\!\!{\sc cycle}\!\!&\!\!.0102 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0100 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0101 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0099 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0100 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0100 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & ---&\!\!.0101 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{.0099} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0105 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! \\
\hline
\!\!{\sc higgs}\!\!&\!\!0.883 {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!0.822 {\tiny $\pm$\hspace*{0.2ex}.022}\!\!&\!\!0.808 {\tiny $\pm$\hspace*{0.2ex}.021}\!\!&\!\!0.845 {\tiny $\pm$\hspace*{0.2ex}.022}\!\!&\!\!\textbf{0.804} {\tiny $\pm$\hspace*{0.2ex}.020}\!\!&\!\!0.812 {\tiny $\pm$\hspace*{0.2ex}.022}\!\!&\!\!0.856 {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!0.824 {\tiny $\pm$\hspace*{0.2ex}.024}\!\!&\!\!0.830 {\tiny $\pm$\hspace*{0.2ex}.024}\!\!&\!\!0.902 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc letter}\!\!&\!\!.0359 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0348 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0340 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0354 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!\textbf{.0339} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0342 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0352 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0343 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0344 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0451 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc magic}\!\!&\!\!0.399 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.391 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.396 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.390 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!\textbf{0.389} {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!0.395 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.389 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!0.393 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.393 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.401 {\tiny $\pm$\hspace*{0.2ex}.008}\!\! \\
\hline
\!\!{\sc pendigits}\!\!&\!\!.0075 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0072 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0073 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0071 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0071 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0071 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!\textbf{.0070} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0071 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0071 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0079 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc satimage}\!\!&\!\!.0490 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0465 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0463 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0476 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0464 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!\textbf{.0458} {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0478 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0470 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0465 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0488 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc seismic}\!\!&\!\!0.308 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.299 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.299} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.300 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.299 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.299 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.300 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.299 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.299 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.311 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc shuttle}\!\!&\!\!\textbf{.0041} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0046 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0042 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0054 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0046 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0044 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0066 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0055 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0049 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0046 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! \\
\hline
\!\!{\sc thyroid}\!\!&\!\!\textbf{0.155} {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.158 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.162 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.156 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.162 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.164 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.156 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.159 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.162 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.175 {\tiny $\pm$\hspace*{0.2ex}.008}\!\! \\
\hline
\!\!{\sc updrs}\!\!&\!\!.0126 {\tiny $\pm$\hspace*{0.2ex}.012}\!\!&\!\!\textbf{.0099} {\tiny $\pm$\hspace*{0.2ex}.006}\!\!&\!\!.0136 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!.0333 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!.0172 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!.0174 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!.0346 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!.0153 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!.0112 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!.0537 {\tiny $\pm$\hspace*{0.2ex}.005}\!\! \\
\hline 
\end{tabular}



==> scenario_experiments.tex <==
\begin{tabular}{|r|r|r|r|r|r|r|r|r|}
\hline
Data Set &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\!& \!best Arch.\!& Gauss \\
\hline
\!\!{\sc bank}\!\!&\!\!\textbf{0.117} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{0.117} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{0.117} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{0.117} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{0.117} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{0.117} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{\textit{0.117}} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{0.117} {\tiny $\pm$\hspace*{0.2ex}.000}\!\! \\
\hline
\!\!{\sc cadata}\!\!&\!\!1.845 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!1.787 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!\textbf{1.679} {\tiny $\pm$\hspace*{0.2ex}.018}\!\!&\!\!1.846 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! & ---&\!\!4.809 {\tiny $\pm$\hspace*{0.2ex}9.36}\!\!&\!\!\textbf{\textit{1.679}} {\tiny $\pm$\hspace*{0.2ex}.018}\!\!&\!\!1.870 {\tiny $\pm$\hspace*{0.2ex}.015}\!\! \\
\hline
\!\!{\sc cod}\!\!&\!\!.0393 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0389 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0389 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!\textbf{.0383} {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & ---&\!\!.0385 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0384 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0395 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc covtype}\!\!&\!\!\textbf{0.136} {\tiny $\pm$\hspace*{0.2ex}.007}\!\!&\!\!0.137 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!0.142 {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.139 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.151 {\tiny $\pm$\hspace*{0.2ex}.007}\!\!&\!\!0.145 {\tiny $\pm$\hspace*{0.2ex}.014}\!\!&\!\!\textbf{\textit{0.133}} {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.179 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc cpusmall}\!\!&\!\!1.025 {\tiny $\pm$\hspace*{0.2ex}.022}\!\!&\!\!\textbf{0.995} {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!1.017 {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!1.012 {\tiny $\pm$\hspace*{0.2ex}.014}\!\! & ---&\!\!1.013 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! & ---&\!\!1.030 {\tiny $\pm$\hspace*{0.2ex}.019}\!\! \\
\hline
\!\!{\sc cycle}\!\!&\!\!1.354 {\tiny $\pm$\hspace*{0.2ex}.032}\!\!&\!\!1.321 {\tiny $\pm$\hspace*{0.2ex}.037}\!\! & ---&\!\!\textbf{1.307} {\tiny $\pm$\hspace*{0.2ex}.044}\!\! & --- & --- & ---&\!\!1.365 {\tiny $\pm$\hspace*{0.2ex}.021}\!\! \\
\hline
\!\!{\sc higgs}\!\!&\!\!\textbf{0.318} {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!0.325 {\tiny $\pm$\hspace*{0.2ex}.006}\!\!&\!\!0.343 {\tiny $\pm$\hspace*{0.2ex}.012}\!\!&\!\!0.326 {\tiny $\pm$\hspace*{0.2ex}.019}\!\!&\!\!0.346 {\tiny $\pm$\hspace*{0.2ex}.015}\!\!&\!\!0.341 {\tiny $\pm$\hspace*{0.2ex}.012}\!\!&\!\!\textbf{\textit{0.313}} {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!0.370 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc letter}\!\!&\!\!.0461 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!.0510 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!.0439 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0458 {\tiny $\pm$\hspace*{0.2ex}.006}\!\!&\!\!.0449 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{.0433} {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0434 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0686 {\tiny $\pm$\hspace*{0.2ex}.013}\!\! \\
\hline
\!\!{\sc magic}\!\!&\!\!\textbf{0.352} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{0.352} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{0.352} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{0.352} {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & ---&\!\!\textbf{0.352} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{\textit{0.352}} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{0.352} {\tiny $\pm$\hspace*{0.2ex}.000}\!\! \\
\hline
\!\!{\sc pendigits}\!\!&\!\!\textbf{.0054} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0078 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0057 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0067 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0063 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0055 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! & ---&\!\!\textbf{.0054} {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc satimage}\!\!&\!\!0.171 {\tiny $\pm$\hspace*{0.2ex}0.11}\!\!&\!\!0.186 {\tiny $\pm$\hspace*{0.2ex}.039}\!\!&\!\!0.129 {\tiny $\pm$\hspace*{0.2ex}.015}\!\!&\!\!0.139 {\tiny $\pm$\hspace*{0.2ex}.019}\!\!&\!\!0.130 {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!0.144 {\tiny $\pm$\hspace*{0.2ex}.020}\!\! & ---&\!\!\textbf{.0949} {\tiny $\pm$\hspace*{0.2ex}.006}\!\! \\
\hline
\!\!{\sc seismic}\!\!&\!\!0.280 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!\textbf{0.278} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.281 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!0.280 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.281 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.282 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!\textbf{\textit{0.277}} {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.286 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc shuttle}\!\!&\!\!\textbf{.0031} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0034 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0033 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0032 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! & ---&\!\!.0032 {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!\textbf{\textit{.0031}} {\tiny $\pm$\hspace*{0.2ex}.000}\!\!&\!\!.0032 {\tiny $\pm$\hspace*{0.2ex}.000}\!\! \\
\hline
\!\!{\sc thyroid}\!\!&\!\!.0428 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0417 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0425 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!\textbf{.0411} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0421 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0417 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! & ---&\!\!.0453 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc updrs}\!\!&\!\!.0480 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0620 {\tiny $\pm$\hspace*{0.2ex}.013}\!\!&\!\!.0450 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!\textbf{.0380} {\tiny $\pm$\hspace*{0.2ex}.014}\!\!&\!\!.0600 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!.0398 {\tiny $\pm$\hspace*{0.2ex}.014}\!\! & ---&\!\!.0732 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline 
\end{tabular}



==> table1.tex <==
\begin{tabular}{|r|r|r|r|r|r|r|r|r|}
\hline
Data Set &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!N\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\!& \!best Arch.\!& Gauss \\
\hline
\!\!{\sc bank}\!\!&\!\!\textbf{.0694} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0719 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0722 {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!\textbf{.0699} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0713 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0704 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{\textit{.0680}} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!.0754 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc cadata}\!\!&\!\!31.56 {\tiny $\pm$\hspace*{0.2ex}0.40}\!\!&\!\!29.69 {\tiny $\pm$\hspace*{0.2ex}0.46}\!\!&\!\!\textbf{27.33} {\tiny $\pm$\hspace*{0.2ex}0.71}\!\!&\!\!31.41 {\tiny $\pm$\hspace*{0.2ex}0.56}\!\! & ---&\!\!31.58 {\tiny $\pm$\hspace*{0.2ex}0.78}\!\!&\!\!\textbf{\textit{27.33}} {\tiny $\pm$\hspace*{0.2ex}0.71}\!\!&\!\!32.38 {\tiny $\pm$\hspace*{0.2ex}0.76}\!\! \\
\hline
\!\!{\sc cod}\!\!&\!\!0.170 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!\textbf{0.142} {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.154 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!0.181 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & ---&\!\!0.181 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.142 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!0.188 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc covtype}\!\!&\!\!0.415 {\tiny $\pm$\hspace*{0.2ex}.018}\!\!&\!\!\textbf{0.414} {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!0.426 {\tiny $\pm$\hspace*{0.2ex}.023}\!\!&\!\!0.421 {\tiny $\pm$\hspace*{0.2ex}.019}\!\!&\!\!0.448 {\tiny $\pm$\hspace*{0.2ex}.023}\!\!&\!\!0.432 {\tiny $\pm$\hspace*{0.2ex}.032}\!\!&\!\!\textbf{\textit{0.409}} {\tiny $\pm$\hspace*{0.2ex}.007}\!\!&\!\!0.527 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc cpusmall}\!\!&\!\!9.015 {\tiny $\pm$\hspace*{0.2ex}0.38}\!\!&\!\!\textbf{8.699} {\tiny $\pm$\hspace*{0.2ex}0.22}\!\!&\!\!8.750 {\tiny $\pm$\hspace*{0.2ex}0.28}\!\!&\!\!8.814 {\tiny $\pm$\hspace*{0.2ex}0.25}\!\! & ---&\!\!8.889 {\tiny $\pm$\hspace*{0.2ex}0.25}\!\! & ---&\!\!9.263 {\tiny $\pm$\hspace*{0.2ex}0.29}\!\! \\
\hline
\!\!{\sc cycle}\!\!&\!\!14.45 {\tiny $\pm$\hspace*{0.2ex}0.74}\!\!&\!\!14.24 {\tiny $\pm$\hspace*{0.2ex}0.76}\!\! & ---&\!\!\textbf{13.92} {\tiny $\pm$\hspace*{0.2ex}0.68}\!\! & --- & --- & ---&\!\!14.74 {\tiny $\pm$\hspace*{0.2ex}0.50}\!\! \\
\hline
\!\!{\sc higgs}\!\!&\!\!\textbf{0.819} {\tiny $\pm$\hspace*{0.2ex}.023}\!\!&\!\!0.833 {\tiny $\pm$\hspace*{0.2ex}.013}\!\!&\!\!0.867 {\tiny $\pm$\hspace*{0.2ex}.024}\!\!&\!\!0.832 {\tiny $\pm$\hspace*{0.2ex}.035}\!\!&\!\!0.869 {\tiny $\pm$\hspace*{0.2ex}.025}\!\!&\!\!0.859 {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!\textbf{\textit{0.810}} {\tiny $\pm$\hspace*{0.2ex}.015}\!\!&\!\!0.905 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc letter}\!\!&\!\!5.880 {\tiny $\pm$\hspace*{0.2ex}0.44}\!\!&\!\!5.864 {\tiny $\pm$\hspace*{0.2ex}0.45}\!\!&\!\!5.879 {\tiny $\pm$\hspace*{0.2ex}0.45}\!\!&\!\!\textbf{5.727} {\tiny $\pm$\hspace*{0.2ex}0.30}\!\!&\!\!5.998 {\tiny $\pm$\hspace*{0.2ex}0.23}\!\!&\!\!5.757 {\tiny $\pm$\hspace*{0.2ex}0.30}\!\!&\!\!5.755 {\tiny $\pm$\hspace*{0.2ex}0.33}\!\!&\!\!7.158 {\tiny $\pm$\hspace*{0.2ex}0.31}\!\! \\
\hline
\!\!{\sc magic}\!\!&\!\!0.101 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.100} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.100} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.100} {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & ---&\!\!\textbf{0.100} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{\textit{0.100}} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.103 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc pendigits}\!\!&\!\!0.179 {\tiny $\pm$\hspace*{0.2ex}.015}\!\!&\!\!0.203 {\tiny $\pm$\hspace*{0.2ex}.014}\!\!&\!\!\textbf{0.157} {\tiny $\pm$\hspace*{0.2ex}.016}\!\!&\!\!0.179 {\tiny $\pm$\hspace*{0.2ex}.014}\!\!&\!\!0.164 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!0.159 {\tiny $\pm$\hspace*{0.2ex}.012}\!\! & ---&\!\!0.170 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! \\
\hline
\!\!{\sc satimage}\!\!&\!\!0.914 {\tiny $\pm$\hspace*{0.2ex}0.63}\!\!&\!\!0.910 {\tiny $\pm$\hspace*{0.2ex}0.18}\!\!&\!\!\textbf{0.610} {\tiny $\pm$\hspace*{0.2ex}.045}\!\!&\!\!0.681 {\tiny $\pm$\hspace*{0.2ex}.070}\!\!&\!\!0.639 {\tiny $\pm$\hspace*{0.2ex}.045}\!\!&\!\!0.714 {\tiny $\pm$\hspace*{0.2ex}.042}\!\! & ---&\!\!4.898 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc seismic}\!\!&\!\!0.301 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.298} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.304 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.303 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.304 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.305 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.300 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.318 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc shuttle}\!\!&\!\!.0500 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!\textbf{.0460} {\tiny $\pm$\hspace*{0.2ex}.007}\!\!&\!\!.0713 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!.0519 {\tiny $\pm$\hspace*{0.2ex}.006}\!\! & ---&\!\!.0521 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!.0479 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!.0471 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc thyroid}\!\!&\!\!0.161 {\tiny $\pm$\hspace*{0.2ex}.010}\!\!&\!\!\textbf{0.158} {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.166 {\tiny $\pm$\hspace*{0.2ex}.013}\!\!&\!\!\textbf{0.158} {\tiny $\pm$\hspace*{0.2ex}.009}\!\!&\!\!0.165 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!0.163 {\tiny $\pm$\hspace*{0.2ex}.009}\!\! & ---&\!\!0.195 {\tiny $\pm$\hspace*{0.2ex}.014}\!\! \\
\hline
\!\!{\sc updrs}\!\!&\!\!.0301 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0409 {\tiny $\pm$\hspace*{0.2ex}.011}\!\!&\!\!.0267 {\tiny $\pm$\hspace*{0.2ex}.005}\!\!&\!\!\textbf{.0217} {\tiny $\pm$\hspace*{0.2ex}.012}\!\!&\!\!.0397 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0235 {\tiny $\pm$\hspace*{0.2ex}.011}\!\! & ---&\!\!.0530 {\tiny $\pm$\hspace*{0.2ex}.004}\!\! \\
\hline 
\end{tabular}



==> valtrain_experiments.tex <==
\begin{tabular}{|r|r|r|r|r|r|r|r|}
\hline
Data Set &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}4, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}8, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}2\!\! &\!\!l\hspace*{0.2ex}=\hspace*{0.2ex}16, S\hspace*{0.2ex}=\hspace*{0.2ex}4\!\!& Gauss \\
\hline
\!\!{\sc bank}\!\!&\!\!\textbf{.0682} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0706 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0711 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0683 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0702 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0691 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!.0739 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc cadata}\!\!&\!\!31.09 {\tiny $\pm$\hspace*{0.2ex}0.34}\!\!&\!\!29.42 {\tiny $\pm$\hspace*{0.2ex}0.57}\!\!&\!\!\textbf{27.43} {\tiny $\pm$\hspace*{0.2ex}0.69}\!\!&\!\!31.04 {\tiny $\pm$\hspace*{0.2ex}0.49}\!\! & ---&\!\!31.48 {\tiny $\pm$\hspace*{0.2ex}0.94}\!\!&\!\!31.80 {\tiny $\pm$\hspace*{0.2ex}0.68}\!\! \\
\hline
\!\!{\sc cod}\!\!&\!\!0.154 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!\textbf{0.132} {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.141 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.164 {\tiny $\pm$\hspace*{0.2ex}.004}\!\! & ---&\!\!0.167 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.176 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline
\!\!{\sc covtype}\!\!&\!\!\textbf{0.330} {\tiny $\pm$\hspace*{0.2ex}.020}\!\!&\!\!0.332 {\tiny $\pm$\hspace*{0.2ex}.012}\!\!&\!\!0.348 {\tiny $\pm$\hspace*{0.2ex}.033}\!\!&\!\!0.336 {\tiny $\pm$\hspace*{0.2ex}.024}\!\!&\!\!0.385 {\tiny $\pm$\hspace*{0.2ex}.027}\!\!&\!\!0.352 {\tiny $\pm$\hspace*{0.2ex}.036}\!\!&\!\!0.456 {\tiny $\pm$\hspace*{0.2ex}.008}\!\! \\
\hline
\!\!{\sc higgs}\!\!&\!\!\textbf{0.799} {\tiny $\pm$\hspace*{0.2ex}.021}\!\!&\!\!0.816 {\tiny $\pm$\hspace*{0.2ex}.015}\!\!&\!\!0.850 {\tiny $\pm$\hspace*{0.2ex}.025}\!\!&\!\!0.814 {\tiny $\pm$\hspace*{0.2ex}.035}\!\!&\!\!0.853 {\tiny $\pm$\hspace*{0.2ex}.025}\!\!&\!\!0.839 {\tiny $\pm$\hspace*{0.2ex}.017}\!\!&\!\!0.894 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc letter}\!\!&\!\!5.862 {\tiny $\pm$\hspace*{0.2ex}0.27}\!\!&\!\!5.861 {\tiny $\pm$\hspace*{0.2ex}0.33}\!\!&\!\!5.865 {\tiny $\pm$\hspace*{0.2ex}0.19}\!\!&\!\!\textbf{5.731} {\tiny $\pm$\hspace*{0.2ex}0.29}\!\!&\!\!5.983 {\tiny $\pm$\hspace*{0.2ex}0.27}\!\!&\!\!5.756 {\tiny $\pm$\hspace*{0.2ex}0.21}\!\!&\!\!7.096 {\tiny $\pm$\hspace*{0.2ex}0.31}\!\! \\
\hline
\!\!{\sc magic}\!\!&\!\!0.101 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.101 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.100} {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.100 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! & ---&\!\!0.101 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.103 {\tiny $\pm$\hspace*{0.2ex}.002}\!\! \\
\hline
\!\!{\sc seismic}\!\!&\!\!0.297 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!\textbf{0.294} {\tiny $\pm$\hspace*{0.2ex}.001}\!\!&\!\!0.299 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.298 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.300 {\tiny $\pm$\hspace*{0.2ex}.002}\!\!&\!\!0.301 {\tiny $\pm$\hspace*{0.2ex}.003}\!\!&\!\!0.314 {\tiny $\pm$\hspace*{0.2ex}.001}\!\! \\
\hline
\!\!{\sc shuttle}\!\!&\!\!.0455 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!\textbf{.0404} {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0646 {\tiny $\pm$\hspace*{0.2ex}.008}\!\!&\!\!.0486 {\tiny $\pm$\hspace*{0.2ex}.009}\!\! & ---&\!\!.0465 {\tiny $\pm$\hspace*{0.2ex}.004}\!\!&\!\!.0431 {\tiny $\pm$\hspace*{0.2ex}.003}\!\! \\
\hline 
\end{tabular}


